Empirical Evaluation of PRNU Fingerprint Variation for Mismatched Imaging Pipelines

We assess the variability of PRNU-based camera fingerprints with mismatched imaging pipelines (e.g., different camera ISP or digital darkroom software). We show that camera fingerprints exhibit non-negligible variations in this setup, which may lead to unexpected degradation of detection statistics in real-world use-cases. We tested 13 different pipelines, including standard digital darkroom software and recent neural-networks. We observed that correlation between fingerprints from mismatched pipelines drops on average to 0.38 and the PCE detection statistic drops by over 40%. The degradation in error rates is the strongest for small patches commonly used in photo manipulation detection, and when neural networks are used for photo development. At a fixed 0.5% FPR setting, the TPR drops by 17 ppt (percentage points) for 128 px and 256 px patches.

==> tables/resolutions.tex <==
\begin{table*}[htb!]
\caption{Spatial dimensions (in pixels) of processed images obtained using all pipelines in our dataset}
\label{tab:ISP_Dataset}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
{\color[HTML]{9A0000} }                                  & \multicolumn{13}{c|}{{\color[HTML]{3531FF} \textbf{Camera Processing Pipelines}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \cline{2-14} 
\multirow{-2}{*}{{\color[HTML]{9A0000} \textbf{Camera}}} & {\color[HTML]{3531FF} \textbf{\begin{tabular}[c]{@{}c@{}}Raw Therapee\\ (RawTh)\end{tabular}}} & {\color[HTML]{3531FF} \textbf{Aftershot}} & {\color[HTML]{3531FF} \textbf{\begin{tabular}[c]{@{}c@{}}Lightzone\\ (LightZ)\end{tabular}}} & {\color[HTML]{3531FF} \textbf{DCRaw}} & {\color[HTML]{3531FF} \textbf{LibRaw}} & {\color[HTML]{3531FF} \textbf{Affinity}} & {\color[HTML]{3531FF} \textbf{Luminar}} & {\color[HTML]{3531FF} \textbf{DXO}} & {\color[HTML]{3531FF} \textbf{\begin{tabular}[c]{@{}c@{}}Capture1\\ (C1)\end{tabular}}} & {\color[HTML]{3531FF} \textbf{\begin{tabular}[c]{@{}c@{}}Lightroom\\ (LightR)\end{tabular}}} & {\color[HTML]{3531FF} \textbf{INet}} & {\color[HTML]{3531FF} \textbf{UNet}} & {\color[HTML]{3531FF} \textbf{DNet}} \\ \hline
{\color[HTML]{9A0000} \textbf{Canon EOS 40D}}            & 2594 x 3900                                                                                    & -                                         & 2592 x 3898                                                                                  & 2602 x 3908                           & 2602 x 3908                            & 2602 x 3908                              & 2592 x 3888                             & 2592 x 3888                         & 2592 x 3888                                                                             & 2592 x 3888                                                                                  & 2602 x 3908                          & 2602 x 3908                          & 2602 x 3908                          \\ \hline
{\color[HTML]{9A0000} \textbf{Canon EOS 5D}}             & 2912 x 4378                                                                                    & -                                         & 2910 x 4376                                                                                  & 2920 x 4386                           & 2920 x 4386                            & 2920 x 4386                              & 2912 x 4368                             & 2912 x 4368                         & 2912 x 4368                                                                             & \textbf{Diff. sizes}                                                                         & 2920 x 4386                          & 2920 x 4386                          & 2920 x 4386                          \\ \hline
{\color[HTML]{9A0000} \textbf{Nikon D7000}}              & 3272 x 4940                                                                                    & 3264 x 4928                               & 3270 x 4938                                                                                  & 3280 x 4948                           & 3280 x 4948                            & 3280 x 4948                              & 3264 x 4928                             & 3264 x 4928                         & \textbf{Diff. sizes}                                                                    & 3264 x 4928                                                                                  & 3280 x 4948                          & 3280 x 4948                          & 3280 x 4948                          \\ \hline
{\color[HTML]{9A0000} \textbf{Nikon D90}}                & 2860 x 4302                                                                                    & 2860 x 4290                               & 2858 x 4300                                                                                  & 2868 x 4310                           & 2868 x 4310                            & 2868 x 4310                              & 2848 x 4288                             & 2848 x 4288                         & \textbf{Diff. sizes}                                                                    & 2848 x 4288                                                                                  & 2868 x 4310                          & 2868 x 4310                          & 2868 x 4310                          \\ \hline
\end{tabular}
}
\end{table*}

